End-to-end Learning of Multi-sensor 3D Tracking by Detection

In this paper we propose a novel approach to tracking by detection that can exploit both cameras as well as LIDAR data to produce very accurate 3D trajectories. Towards this goal, we formulate the problem as a linear program that can be solved exactly, and learn convolutional networks for detection as well as matching in an end-to-end manner. We evaluate our model in the challenging KITTI dataset and show very competitive results.

==> content/end_to_end_learning.tex <==
\subsubsection{End to End Learning}
\label{sec:end_to_end_learning}

To learn the model end to end, we separate the computation graph into two parts, one that computes the output of the neural networks on the GPUs and another that solves the LP on the CPU. Particularly, we define the graph in TensorFlow \cite{tensorflow} and solve the LP with Gurobi \cite{gurobi}. While we have to manually define the subgradients of the LP, the rest of the gradients are computed automatically via TensorFlow's automatic differentiation. To speed up training of the DSM, we initialize the networks by briefly pre-training them for their specific task and then train the entire model. While it is possible to train the entire model from scratch, this approach proved to considerably reduce the clock time of training.


==> content/matching_network.tex <==
\section{Matching Network}
\label{sec:matching_network}

One of the fundamental tasks in tracking is deciding whether or not two detections in
subsequent frames represent the same object. In this work, we use deep neural networks to learn how to match by exploiting both appearance and spatial information. Towards this goal, we design an architecture where one branch processes the appearance of each detection with a convolutional neural network, while two others consist of feedforward networks dealing with spatial information. The activations of all branches are then fed to a fully connected layer to produce the matching score.

\subsection{Appearance Branch}

To extract appearance features, we employ a siamese appearance network based on VGG16 \cite{vgg16}. Note that in a siamese setup, the networks involved share the same set of weights, this makes the architecture more efficient in terms of memory and also makes intuitive sense since both inputs should be evaluated with respect to the same features.

Note that each detection is resized to an input with dimension $224\times224$. To produce a concise representation of the activations without using fully connected layers, each of the max-pool outputs is passed through a product layer followed by a weighted sum, which produces a single scalar for each max-pool layer. This produces an activation vector of size 5.

The choice of using skip-pooling stems from the intuition that matching should exploit both low-level features (color, most importantly) from the initial layers and higher level features from the posterior layers. If we chose to only use the last max-pool layer we would force the network to retain the low-level features all the way to the end or learn an alternative representation, which is less efficient.

\subsection{Spatial Branch}

To incorporate spatial information into the model, two feedforward networks are used. One takes as input an occupancy grid in bird's eye perspective. The other network takes as input an occupancy grid in front view perspective.

In bird's eye perspective, each 3D detection is projected onto a ground plane, leaving only a rotated rectangle that reflects its occupancy in the world. This encoding produces two binary images of size $180\times200$. The product of the pair of images is taken and flattened to a $36000$ vector, which is then fed to the feedforward network.

Note that since the observer is a mobile platform (an autonomous vehicle, in this case), the coordinate system between two subsequent frames would be slightly shifted since the observed moved in the time elapsed. Since its speed in each axis is known from the IMU data, one can calculate the displacement of the observer between each observation and translate the coordinates accordingly, such that both grids are on the exact same coordinate system. This approach is important to make the system invariable to the speed of the observer.

The front view perspective encodes the rectangular area in the camera occupied by the target. It is the equivalent of projecting the 3D bounding box onto camera coordinates. This produces two images of size $120\times300$. Like with the bird's eye encoding, the product of the images is taken and the result is flattened, also producing a $36000$ vector fed to the feedforward network.

A fully connected layer is a good choice to capture the spatial patterns, since it is known that cars behave in different ways depending on where they are with respect to the ego-car. For instance, a car in front of the observer (in the same lane) is likely to move forward, while cars on the left lane are likely to come towards the ego-car. This information would be lost in a convolutional architecture since it would be spatially invariant.


==> content/scoring_network.tex <==
\subsubsection{Scoring Network}
\label{sec:scoring_network}

Because of GPU memory constraints, it is unfeasible to backpropagate a meaningful mini-batch in terms of tracking through the detector's scoring and proposal networks (note that, however, the math of the model still allows that). To counter this issue, detections are treated as the point of entry to the model and passed through a scoring network to handle false positives. This also allows for optimization in the context of tracking.

Towards this end, we employ an architecture that consists of VGG16's convolutional neural network, shown in \autoref{diag:scoring_architecture}. It uses VGG16 to extract features from the RGB detections, followed by 256 densely connected hidden units. It is trained to produce the detection scores, i.e. measure how likely it is that the RGB detection portrays a vehicle. This proved sufficient in the experimental evaluation.

\begin{figure}[h]
  \centering
  \resizebox{\columnwidth}{!}{%
    \begin{tikzpicture}[-latex',font=\sffamily\bfseries,thick,node distance = 4cm]
    \node [inner sep=0pt] (img1) {\includegraphics[width=.2\textwidth]{det.png}};
    \node [conv, right of=img1] (vgg1) {VGG16 CNN};
    \node [mlp, right of=vgg1] (mlp1) {Feedforward \\ Network (ReLU) \\ 25088x256};
    \node [mlp, right of=mlp1] (mlp2) {Feedforward \\ Network (ReLU) \\ 256x2};
    \node [output, right of=mlp2] (scr) {Score};

    \path [line] (img1) -- (vgg1);
    \path [line] (vgg1) -- (mlp1);
    \path [line] (mlp1) -- (mlp2);
    \path [line] (mlp2) -- (scr);
    \end{tikzpicture}}
\caption{Illustration of the scoring network.}
\label{diag:scoring_architecture}
\end{figure}

 While simple, this architecture makes intuitive sense. Most detectors rely on depth, stereo or pointcloud data for spatial positioning of the bounding boxes, while the scoring of the detection is done via convolution of the RGB patches, which is precisely what this architecture does.

